Position: Let's Strengthen Verifiability If We Can't Enforce Reproducibility

In the field of Machine Learning, many papers contain empirical results supporting claimed statements or illustrating the performance of a proposed method. However, most practitioners know that (1) results are generally hard to reproduce, and increasingly so, (2) code is not often available to do so, and (3) it hinders the development of research. In this position paper, we analyze and quantify these issues, and make concrete proposals to improve result checkability, if not reproducibility. Code and supporting materials are available at https://github.com/giddyyupp/position-enforce-verifiability.

==> sec/XXX_notes.tex <==
\section{NOTES ---------------}

The software license, if any, must be worldwide and no-charge, but it may have restrictions, e.g., regarding the copy, the modification, or the use (e.g., only for non-commercial purposes) of the software.


General structure of the paper
\begin{enumerate}[nosep]
    \item intro, definition ACM, motivation
    \item related effort, ML check list, NeurIPS 2019, CVPR 2026 (logs but for consumption), automated paper reproducibility (paper2code)
    \item barriers to reproducibility: lack of many details (significant effort to fill the gaps with plausible solutions, sensitivity to parameter setting depending on datasets), Code availability: stats and analysis, barriers to code availability + code not enough (reproduced numbers different from paper, TTA, bad practices). 
    \item proposals (addressing case when code not made available) = not to reproduce but at least to show good faith and good practice of original authors: logs, pytorch framework with keys/hashes (server is too long shot), 
    \item incentive (carrot and stick). Carrot: stats of research boost thanks to available code, number citation rules for previous papers/results. Stick: two sections in result tables (verified or not)
    \item alternatives: imposing code, if on wants to be peer-reviewed, then code has to be provided. Otherwise, a report on arxiv is enough.
    \item conclusion
\end{enumerate}


\paragraph{Reimplementing}

Although some people do reimplement some papers they need to compare to, there are so many details

paper2code

\paragraph{Misc}

\begin{itemize}[nosep]
    \item The checking material (data, code or stamp) must be available at the time of the conference. This offers enough time after a submission rush to prepare material.
\end{itemize}

\subsection{Third-party checking server}

Training: option by paying money. Not at the begining, long shot

Forget about variance in inference, but several models could be checked and the results averaged.

ArXiv, OpenReview started small, now very big.

%===========================================================

\subsection{Interesting statistics}

We need to show both that the lack of code is an issue and that the availability of code is a big plus

\begin{itemize}[nosep]
    \item Quantity of:
    \begin{itemize}
        \item papers
        \item papers with full code
        \item papers with inference code + weights (but method could be training free, ask an LLM?)
        \item papers with invalid code (what definition? no executable?)
        \item total and per topic
    \end{itemize}
    \item Correlation between number of citations and code availability
    \item Correlation between number of citations and actual code reuse (as building block)
    \item Quantity of unfulfilled promises of code (or promises that disappear after acceptance)
    % \item Correlation (or not) between oral/poster and code availability?
    % \item stats about code sizes, languages?
    % \item Evaluate code quality? 
\end{itemize}

Questions to LLM with README.md
\begin{itemize}[nosep]
    \item Is the method training-based? / Does the method require specific training?
    \item Is there training code available in the repo?
    \item Is there inference/test code available in the repo?
    \item Are there instructions for training?
    \item Are there instructions for inferring/testing ?
    \item Are weights available for the given method (ignoring weights for other methods)?
    \item What is the category/domain of the method among the following list \{...\}?
    \item Are there unresolved/open github issues regarding the installation or reproducibility of performance? ($\rightarrow$ lowerbound)
\end{itemize}
And we need to do the same "by hand" on a number of papers/repos (100?) to show the answers of the LLM matches enough our own assessment.

Question
\begin{itemize}[nosep]
    \item extend to dataset availability?
\end{itemize}


\textbf{Samet Notes}
\begin{itemize}[nosep]
    \item We are analysing open sourced code since it is the sole display of reproducibility currently. However, we should be careful when stating that all methods must be open sourced to ensure reproducibility, as there are many companies conducting research, and most of the time, it is not acceptable to open source methods and/or weights. In my opinion, we lose our audience if we assert this. Instead, we could direct the audience to our proposed solution, i.e., an independent third-party checker that does not retain any code or data afterwards. To achieve this, we can start with the ideal case: a platform where both the training (maybe?) and inference code (along with model weights) are uploaded, and metrics are calculated by the platform. However, this is not easy to do. Then we can suggest starting small with the bare minimum to ensure that the method's premises hold. Also calculation the metrics with the same implementation is another aspect of reproducibility and brings fairness as well.
    \item Actually, WandB has almost all the features to determine whether a method is actually reproducible or not. However, it is easily cheat-able. One could train a random model to show that GPU utilisation is high, and just submit a smooth training loss curve and nice increasing metrics which are synthetically generated. So, when the researcher has low moral codes, these amazing platforms fail to authenticate the methods. But it is worth mentioning WandB. 
    \item Another point is the SIFT method which basically achieves SOTA on many tasks until CNNs could be re-implemented by the community (OpenSIFT or VLFeat) and this implementation was fine. So it was possible to re-implement even though the methods for sure have some intricate elements the number of variables were limited. Now, with deeper models there are significant number of hyper-parameters which affect the end results. Even the initialisation order of the layers and networks changes the initial weights assigned to each trainable weight or element.
    \item Chat with ChatGPT: \url{https://chatgpt.com/s/t_69619584aef48191acbc9301c7f26bb5}
\end{itemize}


%==================================================


% \clearpage

\subsection{Notes}

Notes:
- Now it is nearly impossible to implement a paper's model by just checking the implementation details as the models the community is using are huge by design. Moreover, it is not possible to describe all the intricate details related to the implementation in the paper.   

Lots of ideas discussed in the previous editions of the Workshop on Reproducible Research in Pattern Recognition (RRPR), cf. \url{https://tc22-team.github.io/rrpr2026/previousEditions.html}. See Invited Talks and Reproducible Research Frameworks in
\begin{itemize}
    \item RRPR 2016 (\url{https://link.springer.com/book/10.1007/978-3-319-56414-2#toc})
    \item RRPR 2018 (\url{https://link.springer.com/book/10.1007/978-3-030-23987-9})
    \item RRPR 2020 (\url{https://link.springer.com/book/10.1007/978-3-030-76423-4})
\end{itemize}


Subjects in the calls of RRPR but possibly on the edge of the topic
\begin{itemize}
    \item Potential parameter influence for the result quality (criteria to choose them)
    \item Potential known limitations (or difficult cases)
\end{itemize}

See also Paper2Code \url{https://arxiv.org/pdf/2504.17192}

\paragraph{Algorithm:}
\begin{itemize}[topsep=0pt]
\item Assumption: the method solves a task and is evaluated using some input data and expected output.
\item If the requirements below are not met, then the authors of a new paper are allowed to put the cited results in a separate section of their own result tables with the title "Unchecked results".
\item If the task is "standard":
\begin{itemize}
    \item If the method is evaluated on data for which ground truth is publicly available (ex.\ validation set), then either the code has to be publicly available (possibly with specific licenses) and operational (no unsolved issues), or a server capable of answering processing requests has to be made available (possibly with limits on the input data size, though at least as large as the evaluation set).
    \begin{itemize}
        \item If the code or data are not publicly available, then the results are considered as unchecked. The data when the code is unavailable \emph{has to} be cited.  
        \item If there are issues for operating the code (incomplete code, incomplete data, installation issue?, what else) that are not solved after XXX months, then the code is considered as unchecked and the new paper \emph{has to} refer to the unsolved issue.
    \end{itemize}
    \item If the method is evaluated on data for which the ground truth is not publicly available (e.g., test data for some datasets and tasks) but can be checked on a benchmark server, then the results should appear in the leaderboard of the benchmark.
\end{itemize}    
\item If the task is not standard
    \begin{itemize}
    \item If the task is to learn from a fraction of a dataset
    \begin{itemize}
        \item Then that fraction must be documented 
    \end{itemize}
    \item If the task is a generation task
    \begin{itemize}
        \item 
    \end{itemize}
    \item 
    \end{itemize}

\end{itemize}

\paragraph{Bad solutions:}
\begin{itemize}[nosep]
    \item shuffling the input data: a hash table is enough to cheat and provide expected results.
    \item altering the data (slightly modifying some pixels or points): it is difficult to measure what would be the impact of modifying the input data, even if the change is small.
\end{itemize}

\paragraph{Concerns to (ideally) address:}
\begin{itemize}[nosep]
    \item knowing the ground truth
    \item training on other (more) data than said
    \item selecting a well-trained model or checkpoint based on some external knowledge
    \item actual code more complex than what is described in the paper
\end{itemize}

Is there a reproducibility crisis?
\url{https://www.nature.com/news/polopoly_fs/1.19970!/menu/main/topColumns/topLeftColumn/pdf/533452a.pdf}
Only stats for survey (interviews)

Forks and stars not good metrics: repos without code may have thousands of stars.

IN "RePro: Leveraging Large Language Models for Semi-Automated
Reproduction of Networking Research Results" (\url{}), For
Reproduction of Networking Research Results" (\url{https://arxiv.org/pdf/2509.21074}), For
instance, even in top-tier conferences such as SIGCOMM and
NSDI, only 40.15% of papers published in the last decade
have been accompanied by open-source implementations. Unofficial, third-party reproductions are even scarcer [4], and
private code sharing is often precluded by factors such as
patents or commercial interests. See also their Section 3.1.

% SciReplicate-Bench: Benchmarking LLMs in Agent-driven Algorithmic Reproduction from Research Papers
% https://arxiv.org/pdf/2504.00255




